Learning Optimal Decision Making for an Industrial Truck Unloading Robot using Minimal Simulator Runs

Consider a truck filled with boxes of varying size and unknown mass and an industrial robot with end-effectors that can unload multiple boxes from any reachable location. In this work, we investigate how would the robot with the help of a simulator, learn to maximize the number of boxes unloaded by each action. Most high-fidelity robotic simulators like ours are time-consuming. Therefore, we investigate the above learning problem with a focus on minimizing the number of simulation runs required. The optimal decision-making problem under this setting can be formulated as a multi-class classification problem. However, to obtain the outcome of any action requires us to run the time-consuming simulator, thereby restricting the amount of training data that can be collected. Thus, we need a data-efficient approach to learn the classifier and generalize it with a minimal amount of data. A high-fidelity physics-based simulator is common in general for complex manipulation tasks involving multi-body interactions. To this end, we train an optimal decision tree as the classifier, and for each branch of the decision tree, we reason about the confidence in the decision using a Probably Approximately Correct (PAC) framework to determine whether more simulator data will help reach a certain confidence level. This provides us with a mechanism to evaluate when simulation can be avoided for certain decisions, and when simulation will improve the decision making. For the truck unloading problem, our experiments show that a significant reduction in simulator runs can be achieved using the proposed method as compared to naively running the simulator to collect data to train equally performing decision trees.

==> old-content.tex <==
\section{Introduction}
Many robotics applications require planning and decision making based on what the robot observes in order to complete a task. In this article we use the problem of truck robotic unloading as a motivating application, which is also a good representative of the class of problems that involves decision making for manipulation with highly-complex multi-body interactions. \autoref{fig:motivating-problem} shows an industrial truck unloading robot and cardboard boxes inside the truck that needs to be unloaded. The robot has two end effectors, one is fixed to the base of the robot and can sweep boxes from the floor, and another suspended with an arm and can pick boxes using a plunger mechanism. The terms ``planning'' and ``decision-making'' can carry wide range of meanings. To clarify, in this context, we use ``decision-making'' refers to deciding high-level tasks such as whether the robot decides to sweep boxes from the floor or pick boxes using the arm, and also to decide the pick location. Further, we use ``planning'' to mean determination of the sequence of actions that the robot actuator should take in order to perform a task decided by the high-level strategy. For example, given a specific pick location, a planner provides a sequence of actions for the robot's arm such that it attempts to pick boxes from that specified location while maintaining constraints such as actuator limits, obstacle avoidance etc. This application has also been studied in our prior work \cite{islam2020planning,kim2019pomhdp}, and in this work we present an alternate approach to high-level decision making to solve the problem, and generalize the proposed algorithm to the class of problems it belongs to.

\begin{figure}[t!]
	\centering
	\hfill%
	\includegraphics[width=0.5\columnwidth]{truck-unload}\hfill%
	\includegraphics[width=0.5\columnwidth]{tu-trailer}\hfill%
	\hfill%
	\caption{\small \textbf{Left}: The industrial truck unloading robot. \textbf{Right}: Cardboard boxes inside a truck with the robot facing them.}
	\label{fig:motivating-problem}
\end{figure}

\section{Preliminaries}
We extend our prior work \cite{islam2020planning}. First we present a comparison between this and our prior work, and then discuss other related literature. The truck-unloading problem we study here shares the same challenges faced by \cite{islam2020planning}. The first challenge is attributed to partial-observability of the box states as it is impractical to know the exact pose of each box in the trailer using sensors onboard the robot. Our prior work assumed that the ground-truth pose of each box was available, whereas in the proposed method, we do not make such an assumption, and the high-level decision making is purely based on what a robot c an practically observe with its onboard sensors. Like the previous work, we also assume that the mass and size of the boxes are not known, however in this work we make a reasonable assumption that they belong to same distribution which is used both during training and during operation. 

The second challenge is related to optimal decision making in the class of problems we consider here. The truck unloading problem involves complex multi-body interaction between the boxes, the robot and the truck walls. Even a slight change in interaction may lead to a very different state for the boxes after the action finishes. For any decision-maker, in order to determine a optimal sequence of high-level tasks such as pick or sweep, that would unload the truck, an accurate knowledge of the transition model is required. A transition model specifies the resulting state of the boxes when a high-level task is performed by the robot on an initial state. The resulting state can also be a distribution of states, in which case a common approach is to plan in the belief space \cite{platt2010belief}. Also, some problems that belong to the described class of problems, might require sequential decision making, which means that for optimal performance, the decisions made in the past affects the decisions to be taken in the future. Thus an optimal algorithm would attempt to maximize the \textbf{cumulative reward}. Even with the Markov assumption that the optimal decision only depend on the current observation, the action that is taken now determines the observation for the next iteration, and hence affects the optimal decision for that iteration. For such sequential decision making problem with partial-observability and model uncertainty, a common approach is to frame the problem as a Partially Observable Markov Decision Process (POMDP) \cite{kaelbling1998planning,kochenderfer2015decision}. The truck unloading problem is also a sequential decision making problem, and due to complex interaction between the robot and the boxes, the transition model specifies a distribution over the states. Now, such complex multi-body interactions are hard to model using analytical functions, and thus, a common approach is to use a simulator to perform the action multiple times to capture the distribution of resulting states. \cite{kim2019pomhdp} presents an algorithm named as Partially Observable Multi-Heuristic Dynamic Programming (POMHDP) that solves the POMDP problem in belief space, and utilizes a simulator to estimate the distribution of states. Our prior work was based on this algorithm. While in theory \cite{kim2019pomhdp} presents a principled solution to the class of problems we are interested in by accounting for partial-observability, model uncertainty and sequential decision making, however in our prior work \cite{islam2020planning}, we observed that due to computational limitations, an implementation of the algorithm suffers to utilize the benefits of the principled approach in practice. For example, the truck unloading problem requires a high-fidelity simulator to simulate the complex dynamics of the robot and boxes, and thus each simulator run takes approximately 10 minutes (more details in \autoref{experiments}). Since an explicit transition model is not available, \cite{kim2019pomhdp} uses a particle representation of the belief space, and hence requires many particles (simulator runs) for a reasonably accurate representation. In practice, due to computational limitations, only a few particles are used which leads to inaccurate transition model, and which further leads to a sub-optimal plan. Further, due to \textit{curse of history} and \textit{curse of dimentionality}, in practice a POMDP is solved only up to a certain horizon, making the plan only locally optimal up to that horizon. In summary, due to practical limitations, regardless of POMHDP being asymptotically optimal, the sequence of high-level tasks may be far from global optimality, and without a method to evaluate how sub-optimal the sequence is.

In this work, we therefore propose an algorithm which maximizes the \textbf{immediate reward} as opposed to the cumulative reward, but allows a feasible implementation even under practical limitations. We present this as an alternative to an algorithm that attempts to maximize the cumulative reward and make a case for practical feasibility. Given that the problem involves sequential decision making, maximizing the immediate reward does not guarantee global optimality w.r.t.\ cumulative reward unless the problem has a submodular structure \cite{corah2019distributed,jaleel2018real}. Now to maximize for immediate reward, the decision making problem reduces to a classification problem. Given what the robot has observed, it needs to specify a high-level action among a set of discrete actions, that the robot should take in order to maximize the immediate-reward. To train a classifier, one approach is to first collect a large dataset. However, we one major limiting factor is the cost associated with collecting a single data point. As described in \autoref{problem-formulation}, collecting one data point means running multiple high-level tasks on the robot either in simulation or in real-world, thus there is a large cost associated with collecting a data point. Our main contributions are two fold: 1) a rejection sampling based algorithm that relies on statistical guarantees to minimize the number of data points required to learn an optimal decision tree, and 2) a case study of the algorithm applied to the truck unloading problem.

\section{Problem Formulation}
\label{problem-formulation}


\section{Algorithmic Framework}

\subsection{Optimal Decision Tree}

\subsection{Action Elimination}

\subsection{Feature Selection}

\section{Experiments and Results}
\label{experiments}
